BlockChain I/O: Enabling Cross-Chain Commerce

Blockchain technology enables secure tokens transfers in digital marketplaces, and recent advances in this field provide other desirable properties such as efficiency, privacy, and price stability. However, these properties do not always generalize to a setting across multiple independent blockchains. Despite the growing number of existing blockchain platforms, there is a lack of an overarching framework whose components provide all of the necessary properties for practical cross-chain commerce. We present BlockChain I/O to provide such a framework. BlockChain I/O introduces entities called cross-chain services to relay information between different blockchains. The proposed design ensures that cross-chain services cannot violate transaction safety, and they are furthermore disincentivized from other types of misbehavior through an audit system. BlockChain I/O uses native stablecoins to mitigate price fluctuations, and a decentralized ID system to allow users to prove aspects of their identity without violating privacy. After presenting the core architecture of BlockChain I/O, we demonstrate how to use it to implement a cross-chain marketplace and discuss how its desirable properties continue to hold in the end-to-end system. Finally, we use experimental evaluations to demonstrate BlockChain I/O's practical performance.

==> sec/analysis.tex <==
\subsection{Atomicity}

\begin{itemize}
\item both the winning customers and vendors need to agree to final commit -- as such, non-compliant CC-SVCs can at most violate liveness, not safety
\item at least one CC-SVC required for liveness
\item without the requirement that the winning bidder commits, the auctioneer can 
\item additional security: final commit vote also signed by bidder, which allows the bidder to back out at the last moment
\item trivial aborts can be disincentivized through \textit{premiums} \cite{engel2021failure}
\end{itemize}

\subsection{Pseudonymity}

\subsection{Stablecoin Support}

\subsection{Fairness}


\begin{itemize}
\item misbehavior by CC-SVCs is detectable
\end{itemize}

\subsection{Generality}

\subsection{Efficiency}

\begin{itemize}
\item at least one honest CC-SVC required
\end{itemize}

==> sec/digital_identities.tex <==

\subsection{Entities}
We leverage the zero-knowledge proofs \cite{anoncredstheory} based framework of Hyperledger AnonCreds \cite{anoncreds} for DIDs that represent attribute information. The logical entities involved in the creation and verification of DIDs are as follows. 

 {\textit{Holder}: Any entity which is trying to establish its credentials can be a holder -- e.g., in the cross-chain marketplace, this would typically be a vendor or bidder.}
 
 {\textit{Issuer}: Issuers are entities who are responsible for generating valid schema and credential definitions for holders. In cross-chain applications, they may be any pre-specified trusted organization.
 Issuers themselves are identified using so-called \textit{issuer identifiers}, which are a form of DIDs.
 Accommodating arbitrary entities as issuers makes the approach decentralized -- in effect, issuers have an analogous role to that of certificate authorities in the Web PKI, and DIDs and issuer identifiers can be seen as the analogues of end-entity and intermediate certificates.}
 
 {\textit{Verifier}: The verifier communicates with the VDR for each action and with the \textit{Registration Smart Contract} (RSC) module of \pie where the verifier is notified through an event listing action. The verifier validates the schema identity, credential definition identity, and the DID of the respective holder, and forwards an ECDSA (Elliptic Curve Digital Signature Algorithm) based signed hashed transaction that indicates validation of the DID, along with VC information, to the RSC for acceptance or rejection of the respective holder. }
 
 {\textit{Verifiable data registry} (VDR): Hyperledger AnonCreds is used as a VDR to verify and store the DIDs, schema information, credential definition identity, revocation list for future reference and validation of VCs.}
 
 {\textit{Registration Smart Contract} (RSC): This module realizes the integration of AnonCreds with \blockx and is used to communicate with the credential holders or verifiers. It validates the DID, 160-bit hashed address information and VC of the holder during registration and validates the signed hashed information regarding the holder received from the verifier.} \Cref{fig:anoncreds} depicts the interactions, which, in effect, also require cross-chain communication given that AnonCreds itself is built using the Hyperledger framework.

%{For successful implementation of Hyperledger AnonCreds in this scheme, AnonCreds specification V 1.0 is considered associated with Hyperledger Indy (for management of participant’s pools in JSON-LD format and used as (.txn) file) and implemented in Ubuntu Linux platform version 18.04.4 LTS bionic.}

\begin{figure}[tp!]
\centering
\includegraphics[width=\linewidth]{fig/Figure3_3.pdf}
\caption{\pie and AnonCreds integration \label{fig:anoncreds}} 
\end{figure}

\begin{comment}
\subsection{DID Structure}
During communicating with Registration Smart Contract,  following attributes/schemes are considered by Hyperledger AnonCreds for implementation of the DIDs and shown in Figure \ref{fig:anoncreds} as below:

\begin{itemize}
    \item {W3C recommended zero knowledge scheme and idemix technologies are considered to maintain the anonymous identities of the participants (DID) and public but restricted cross-chain mechanism is also maintained to make every transaction more secure and robust.}
    \item {A public and reusable template is considered as “Schema”, utilized for this scheme to gather holder’s secret credentials by the issuer and forward it to VDR. Moreover, the numbers of holders are also restricted using “maxCredNum” attributes in AnonCreds schema.}
    \item {Using Credential Definition generated based on Schema that helps Issuers to issue AnonCreds credentials for holders and verifiers to verify credentials presented by holders.}
    \item {\textit {Canonicalization encrypted format}: This inbuilt encryption mechanism of AnonCreds is used to generate DIDs and credential information in a secure encrypted manner so it can be shared during internal communication between participants as 32 bit numerical encrypted structure from attribute information. Later on, the 32-bit information is converted to hashed encrypted information after signing by ECDSA signature scheme by the validator during communication between the “Registration Smart Contract”.}
    
\end{itemize}

\end{comment}

\subsection{DID Creation}
For the generation of pseudonym DIDs, the issuer first has to determine the schema and credential definition for the holder (which can be reused for many users/holders when suitable). To generate credentials, the issuer also has to be verified using its issuer identifier. In this regard, both the issuer and verifier first forward their requests to the system pool to obtain their identifiers, verification keys, and roles as Trust Anchor or Trustee respectively. After obtaining a suitable role (Trust Anchor), the issuer requests the AnonCreds VDR to generate the schema of the holder based on some secret credentials provided by the holder using a predefined reusable template. As a response, a schema ID is returned by AnonCreds VDR. Using this schema ID, the issuer requests the credential definition alongside other information like tag values and type and revocation information for the schema.  Next, a DID is generated internally by the verifier. After getting credential definition information from AnonCreds, the issuer forwards it to the holder. Later on, the holder requests verification of the DID against the credential definition. However, based on validation of such information, the verifier either forwards the DID and credential definition 
 -- in a 32-bit encrypted format called the \textit{canonicalization} format -- 
to the holder if the schema is valid (after getting confirmation from AnonCreds), otherwise it rejects the request.

\subsection{DID Verification}
A conversion mechanism is maintained by the verifier to translate information from the canonicalization format to ECDSA-based signed information while communicating with \pie via the RSC. So, after obtaining the DID and credential definition from the holder as a request to interact with other elements of \blockx and the cross-chain marketplace, it is first forwarded to the RSC along with a 160-bit hashed address of the holder. It is then further validated by the RSC (in turn communicating with the validator and the VDR) against the information maintained by the AnonCreds schema and VCs. If the holder is valid, only then the respective credentials are forwarded along with the DID to the RSC to grant the holder access for further communication with \pie, otherwise the request is rejected.


\begin{comment}
\subsection{Example: Use Cases}

Such type of DID based scheme is being widely used in several applications now a day like online shopping, vehicle management, very confidential customer for engagements, maintenance of transferable skills for secure credentials, user-driven cross-platform for sharing of information, supply chain management with pseudonymity,Public authority identity credentials (eIDAS), maintenance of permanent digital residential card, etc. Another use case may be considered for job applicants where the applicant can apply for a job using valid DID as well as VC in online decentralized blockchain network and the job seekers can verify such credentials after communicating with the issuer (University) for the validation of the VC against the DID. 
\end{comment}

==> sec/reputation_system.tex <==
As discussed in \Cref{sec:system_architecture}, information about user transactions on different chains are relayed by CC-SVCs who are disincentivized from misbehaving through an audit system.
In this section, we discuss methods to detect three different forms of misbehavior and prove it to the governance layer. 

% As we saw in \Cref{sec:reputation_systems}, several approaches in the literature exist that 

In the following, we assume the existence of a universal \textit{clock} such that the difference between each block's timestamp and the universal clock never exceeds a maximum value $\Delta>0$. As we discuss later, this assumption removes ambiguity about when listings are concluded, or when a cross-chain reputation score is valid. This assumption is more realistic for some blockchain platforms than for others -- e.g., Bitcoin's block timestamps are only loosely related to real-world times \cite{szalachowski2018short}, whereas in Ethereum's proof-of-stake protocol (post-2022) the timestamps are strictly enforced by the protocol as new blocks are created precisely once every 12 seconds.

\subsection{Misrepresenting a Deal Outcome}

The outcome of a deal should follow the execution logic specified by the creator: e.g., in a first-price open-bid auction, the asset should go to the user who issued the highest bid. It can be profitable for a CC-SVCs to deviate from this logic, e.g., because it received an off-chain bribe from the second-highest bidder. 

To prove that a CC-SVC has misbehaved, ...

\subsection{Misrepresenting a DID or Score}

In \blockx, deals can require that participants in a cross-chain deal satisfy certain attributes. Since the attribute information is typically on a different blockchains than those on which users exchange tokens, information about DIDs must be transmitted and signed by CC-SVCs who act as verifiers. The same is true for a reputation or credit score, which is information 

To prove that a CC-SVC has misbehaved, ...

\subsection{Stalling a Cross-Chain Deal}

If a CC-SVC abandons a cross-chain deal halfway, then this leads to inconvenience to the users as the deal would need to be restarted or an alternative CC-SVC would need to be found.

To prove that a CC-SVC has misbehaved, ...

% \subsection{Audits}

% \tbd{A malicious cross-chain services cannot steal tokens from parties, as each party involved in the final trade must contribute to the commit vote}

% \tbd{Similarly, a faulty or malicious cross-chain service cannot violate liveness, because if one goes offline it should be possible to switch to another cross-chain service to process the listing}

% \tbd{However, a malicious cross-chain service can violate fairness by declaring the wrong party the winner. This can lead to abuse: e.g., if one user bids \$100 and a user on another blockchain bids \$50 for an NFT, then the loser could bribe the cross-chain service with \$10 -- it would be rational for the cross-chain service to accept the bribe if there is no system in place to punish this type of behavior}

% \tbd{In \blockx, auditors can detect this type of misbehavior in retrospect. Upon detection, they should be able to submit proof of the misbehavior to the governance layer. The governance layer should verify the proof of misbehavior, and if found legitimate, it should either slash a deposit by the cross-chain service and reward it to the auditor (and perhaps the vendor and customer involved in the trade), or a demerit point should be added to the cross-chain service.}

% \tbd{Another way in which cross-chain services can misbehave is by misrepresenting the reputation of a vendor to customers}

% \tbd{Again, it should be possible to detect this type of misbehavior and prove it to the governance layer}
